Simulation of scour around arbitrary offshore foundations based on the Volume-of-Fluid method combined with a Bingham model

This paper presents a method for the simulation of scour around arbitrary offshore structures. It is based on the solution of the Reynolds-Averaged-Navier-Stokes equations implemented in the OpenFOAM framework. The sediment is simulated with the help of a Bingham model, which basically models a solid sediment behavior by introducing a very high viscosity. The relative pressure used by the Bingham model is estimated with a new approach based on the solution of a Poisson equation. The position of the sediment surface is calculated with the Volume-of-Fluid approach using a high-resolution scheme. To keep the typical wall characteristics without demanding a fine grid, the common wall functions are transferred to the domain internal sediment walls. Furthermore, additional modifications are applied to model a solid sediment wall inside the solution domain. The new internal wall function implementation is validated with a 2D test case. The results show a very good agreement to common wall functions and a significant improvement compared to its negligence. Furthermore the solver is used to simulate the scour downstream of an apron and the scour around a vertical cylinder in current. The results are compared to experiments presented in the literature and show good agreement. The applicability onto arbitrary structures is demonstrated by applying the solver onto a vertical cylinder with a mudplate. The current development state is able to resolve all important physical flow and scour phenomena. The results also unveil that modeling of the suspension and the treatment of the internal wall need additional attention.

==> chapters/abbreviations.tex <==
%\section*{List of Abbreviations}				%das * sorgt dafür, dass dieses Kapitel nicht im Inhaltsverzeichnis erscheint und ohne Chapter 1 vorweg
\begin{acronym}[YTM]
\setlength{\itemsep}{-\parsep}					% kompakte Darstellung
\renewcommand{\bflabel}[1]{\bfseries{\normalsize{#1}}\hfill}	% Schrift mit den üblichen Serifen
 \acro{BICS}{Blended Interface Capturing Scheme}
 \acro{BRICS}{Blended Reconstructed Interface Capturing Scheme}
 \acro{CBC}{Convective Boundedness Criterion}
 \acro{CDS}{Central Differencing Scheme}
 \acro{CFL}{Courant-Friedrichs-Lewy Number}
 \acro{CFLC}{Courant-Friedrichs-Lewy Condition}
 \acro{CICSAM}{Compressive Interface Capturing Scheme for Arbitrary Meshes}
 \acro{DDS}{Downwind Differencing Scheme}
 \acro{ECBC}{Extended Convective Boundedness Criterion}
 \acro{GDS}{Gamma Differencing Scheme}
 \acro{HRIC}{High-Resolution Interface Capturing}
 \acro{IGDS}{Inter-Gamma Differencing Scheme}
 \acro{lhs}{left hand side}
 \acro{NOCL}{Non-Orthogonal-Corrector Loops}
 \acro{NSE}{Navier-Stokes-Equations}
 \acro{NVA}{Normalized Variable Approach}
 \acro{NVD}{Normalized Variable Diagram}
 \acro{OF}{OpenFOAM}
 \acro{PISO}{Pressure Implicit with Splitting of Operator}
 \acro{RANSE}{Raynolds-Averaged-Navier-Stokes-Equations}
 \acro{SIMPLE}{Semi-Implicit Method for Pressure Linked Equations}
 \acro{rhs}{right hand side}
 \acro{UDS}{Upwind Differencing Scheme}
 \acro{VOF}{Volume-of-Fluid}
\end{acronym}

%----------------------------------------------------------------------------------------------------------------
%Anleitung
%\ac{Abk.}         % fügt die Abkürzung ein, außer beim ersten Aufruf, hier wird die Erklärung mit angefügt
%\acs{Abk.}        % fügt die Abkürzung ein
%\acf{Abk.}        % fügt die Abkürzung UND die Erklärung ein
%\acl{Abk.}        % fügt nur die Erklärung ein

%für den Plural ein zusaätzliches p ans Ende setzen z.B.:
%\acp{Abk.}

%MANUEL ALPHABETISCH SORTIEREN!!!!!!!!!

==> chapters/bibliography.tex <==
\section{References}
\label{References} 

\bibliography{Verzeichnis1}{}
\bibliographystyle{plain}




% \begin{thebibliography}{00}
% %WICHTIG NUMERICAL ORDER!!!!!!
% %-----------------------------------------------------------------------------------------------------------
% %-----------------------------------------------------------------------------------------------------------
% \bibitem{Amoudry2009}
% Amoudry, L.O. and Lie, P.L.-F.,
% Two-dimensional, two-phase granular sediment transport model with applications to scouring downstream of an apron,	
% \textit{Coastal Engineering},
% (2009),
% \textbf{56}(7):693--702.
% %-----------------------------------------------------------------------------------------------------------
% \bibitem{Breusers1965}
% Breusers, H.N.C.,
% Conformity and time scale in two-dimensional local scour,	
% \textit{Delft Hydraulics Laboratory},
% (1965),
% \textbf{40}.
% %-----------------------------------------------------------------------------------------------------------
% \bibitem{Breusers1967}
% Breusers, H.N.C.,
% Time scale of two-dimensional local scour,	
% \textit{Proc. 12th IAHR Congress},
% Ft. Collins,
% (1967),
% \textbf{3}:275--282.
% %-----------------------------------------------------------------------------------------------------------
% %Book
% \bibitem{Breusers1991}
% Breusers, H.N.C. and Raudkivi, A.J.,
% Scouring,	
% \textit{A.A. Balkema},
% Rotterdam,
% (1991),
% %-----------------------------------------------------------------------------------------------------------
% \bibitem[Cheng et al. (2017)]{Cheng2017}
% Cheng, Z., Hsu, T. and Calantoni, J.,
% SedFoam: A multi-dimensional Eulerian two-phase model for sediment transport and its application to momentary bed failure,	
% \textit{Coastal Engineering},
% (2017),
% \textbf{119}:32--50.
% %-----------------------------------------------------------------------------------------------------------
% \bibitem[Graf et al. (2016)]{Graf2016}
% Graf, K., Meyer, J., Renzsch, H.,
% Prediction and optimization of aerodynamic and hydrodynamic forces and boat speed of foiling catamarans with a wing sail and a jib,
% In: Society of Naval and Marine Engineers (Hg.).
% The Twenty-Second Chesapeake Sailing Yacht Symposium: CSYS, March 18-19,
% 2016, Annapolis, Maryland, USA. [Jersey City, N.J.]: Society of Naval and Marine Engineers; 2016.
% %-----------------------------------------------------------------------------------------------------------
% % Graf K, Meyer J, Renzsch H, Preuß C. Investigation of modern sailing yachts using a new free-surface RANSE code. In: Cite de la Voile Eric Taberly and Naval Academy Research Institute. Innovation in high performance sailing yachts (INNOV'SAIL 2017): International conference, 28 June - 30 June 2017, Lorient, France: Lorient / France: Cite de la Voile Eric Taberly and Naval Academy Research Institute; 2017.
% %-----------------------------------------------------------------------------------------------------------
% \bibitem{Jacobsen2012}
% Jacobsen, N.G., Fuhrman, D.R. and Fresd{\o}e, J.,
% A wave generation toolbox for the open-source CFD library: OpenFOAM{\textregistered},	
% \textit{International Journal for Numerical Methods in Fluids},
% (2012),
% \textbf{70}:1073--1088.
%  %-----------------------------------------------------------------------------------------------------------
% \bibitem{Higuera2013}
% Higuera, P., Lara, J.L. and Losada, I.J.,
% Realistic wave generation and active wave absorption for Navier-Stokes models: Application to OpenFOAM{\textregistered},	
% \textit{Coastal Engineering},
% (2013),
% \textbf{71}:119--134.
% %------------------------------------------------------------------------------------------------------------
%  \bibitem{HirtVOF1981}
%  Hirt, C.W. and Nichols, B.D.,
% Volume of Fluid (VOF) Method for the Dynamics of Free Boundaries,	
% \textit{Journal of Computational Physics},
% (1981)
% \textbf{39}:201--225.
%  %-----------------------------------------------------------------------------------------------------------
% \bibitem{QueuteyDR2007}
% Queutey, P. and Visonneau, M.,
% An interface capturing method for free-surface hydrodynamic flows,	
% \textit{Computers $\&$ Fluids},
% (2007),
% \textbf{36}:1481--1510.
%  %-----------------------------------------------------------------------------------------------------------
% \bibitem{WackersBRICS2010}
% Wackers, J., Koren, B., Raven, H.C., van der Ploeg, A., Starke, A.R., Deng, G.B., Queutey, P., Visonneau, M., Hino, T. and Ohashi, K.,
% Free-surface viscous flow solution methods for ship hydrodynamics,	
% \textit{Archives of Computational Methods in Engineering},
% (2010),
% \textbf{18}:1--41.
% %-----------------------------------------------------------------------------------------------------------
% \bibitem{Soeding2001}
% Soeding, H.,
% How to integrate free motion of solids in fluids,
% \textit{4th Numerical Towing Tank Symposium},
% Hamburg-Germany,
% (2001).
%  %-----------------------------------------------------------------------------------------------------------
% \bibitem{Meyer2016}
% Meyer, J., Renzsch, H., Graf, K. and Slawig, T.,
% Advanced CFD-Simulations of free-surface flows around modern sailing yachts using a newly developed OpenFOAM solver,	
% \textit{The 22nd Chesapeake Sailing Yacht Symposium},
% Annapolis-Maryland,
% (2016).
%  %-----------------------------------------------------------------------------------------------------------
% \bibitem{Choi2009}
% Choi, J and Yoon, S.B.,
% Numerical simulations using momentum source wave-maker applied to RANS equation model,	
% \textit{Coastal Engineering},
% (2009),
% \textbf{56}:1043--1060.
%  %-----------------------------------------------------------------------------------------------------------
% \bibitem{Park1999}
% Park, J.C., Kim, M.H. and Miyata, H.,
% Fully non-linear free-surface simulations by a 3D viscous numerical wave tank,	
% \textit{International Journal for Numerical Methods in Fluids},
% (1999),
% \textbf{29}:685--703.
%  %-----------------------------------------------------------------------------------------------------------
% \bibitem{PericR2016}
% Peri\'{c}, R. and Abdel-Maksoud, M.,
% Reliable Damping of Free Surface Waves in Numerical Simulations,	
% \textit{Ship Technology Research},
% (2016),
% \textbf{63}.
%  %-----------------------------------------------------------------------------------------------------------
% \bibitem{PericR2013}
% Peri\'{c}, R.,
% Internal generation of free surface waves and application to bodies in cross sea, MSc Thesis,	
% \textit{Schriftenreihe Schiffbau},
% Hamburg University of Technology,
% Hamburg-Germany,
% (2013).
%  %-----------------------------------------------------------------------------------------------------------
% \bibitem{Ursell1960}
% Ursell, F., Dean, R.G. and Yu, Y.S.,
% Forced small-amplitude water waves: a comparison of theory and experiment,	
% \textit{Journal of Fluid Mechanics},
% (1960),
% \textbf{7}:33--52.
% %-----------------------------------------------------------------------------------------------------------
% 
% 
% \end{thebibliography}
